Masses, Revised Radii, and a Third Planet Candidate in the "Inverted" Planetary System Around TOI-1266

Is the population of close-in planets orbiting M dwarfs sculpted by thermally driven escape or is it a direct outcome of the planet formation process? A number of recent empirical results strongly suggest the latter. However, the unique architecture of the TOI-1266 system presents a challenge to models of planet formation and atmospheric escape given its seemingly "inverted" architecture of a large sub-Neptune ($P_b=10.9$ days, $R_{p,b}=2.62\pm 0.11\, \mathrm{R}_{\oplus}$) orbiting interior to that of the system's smaller planet ($P_c=18.8$ days, $R_{p,c}=2.13\pm 0.12\, \mathrm{R}_{\oplus}$). Here we present revised planetary radii based on new TESS and diffuser-assisted ground-based transit observations, and characterize both planetary masses using a set of 145 radial velocity measurements from HARPS-N ($M_{p,b}=4.23\pm 0.69\, \mathrm{M}_{\oplus}, M_{p,c}=2.88\pm 0.80\, \mathrm{M}_{\oplus}$). Our analysis also reveals a third planet candidate ($P_d=32.3$ days, $M_{p,d}\sin{i} = 4.59^{+0.96}_{-0.94}\, \mathrm{M}_{\oplus}$), which if real, would form a chain of near 5:3 period ratios, although the system is likely not in a mean motion resonance. Our results indicate that TOI-1266 b and c are among the lowest density sub-Neptunes around M dwarfs and likely exhibit distinct bulk compositions of a gas-enveloped terrestrial ($X_{\mathrm{env},b}=5.5\pm 0.7$%) and a water-rich world (WMF$_c=59\pm 14$%), which is supported by hydrodynamic escape models. If distinct bulk compositions are confirmed through atmospheric characterization, the system's unique architecture would represent an interesting test case of inside-out sub-Neptune formation at pebble traps.

==> priors.tex <==
\begin{table}
  \centering
  \caption{Joint light curve and RV model parameter priors\label{tab:priors}}
  \begin{tabular}{lc}
    \hline
    Parameter & Fiducial Model Prior \\
    \hline
    \multicolumn{2}{c}{\emph{Stellar parameters}} \\
    $R_\star$ [$R_{\odot}$] & $\mathcal{N}(0.436,0.013)$ \\
    $M_\star$ [$M_{\odot}$] & $\mathcal{N}(0.431,0.020)$ \\
    \multicolumn{2}{c}{\emph{Light curve parameters}} \\
    $f_{0,T}$ & $\mathcal{U}(-\inf,\inf)$ \\
    $\ln{s^2}$ [ppt$^2$] & $\mathcal{N}(\ln{\text{var}(f_{\text{TESS}})},1)$ \\
    $u_{1,\mathrm{TESS}}$ & $\mathcal{U}(0,1)$ \\
    $u_{2,\mathrm{TESS}}$ & $\mathcal{U}(0,1)$ \\
    $\ln{\sigma}$ [ppt] & $\mathcal{N}(\ln{\text{median}(\sigma_{f_{\text{TESS}}})},1)$  \\
    $\ln{\rho}$ [days] & $\mathcal{N}(50,10)$ \\
    \multicolumn{2}{c}{\emph{RV parameters}} \\
    $\gamma_{\rm RV}$ [m/s] & $\mathcal{U}(-41615,-41595)$  \\
    $\ln{s}_{\rm RV}$ [m/s] & $\mathcal{U}(-3,3)$ \\
    $\ln{\Sigma}$ [m/s] & $\mathcal{U}(-3,3)$ \\
    $P_{\text{rot}}$ [days] & $p(P_{\text{rot}}\vert \text{dLW})^\dagger$ \\
    $\ln{Q_0}$ & $p(\ln{Q_0}\vert \text{dLW})^\dagger$ \\
    $\ln{dQ}$ & $p(\ln{dQ}\vert \text{dLW})^\dagger$ \\
    $\ln{f}$ & $p(\ln{f}\vert \text{dLW})^\dagger$ \\
    \multicolumn{2}{c}{\emph{Planetary parameters}} \\
    $P$ [days] & $\mathcal{U}(-\inf,\inf)$ \\
    $T_{0}$ [BJD-2,457,000] & $\mathcal{U}(-\inf,\inf)$  \\
    $\ln{R_p/R_\star}$ & $\mathcal{U}(-10,0)$ \\
    $b$ & $\mathcal{U}(0,1+R_p/R_\star)$ \\
    $\sqrt{e}\cos{\omega}$ & $\mathcal{U}(-1,1)$ \\
    $\sqrt{e}\sin{\omega}$ & $\mathcal{U}(-1,1)$ \\
    $\ln{K}$ [m/s] & $\mathcal{U}(-3,3)$ \\
    \multicolumn{2}{l}{$^\dagger$ Marginalized posterior distribution from training on our dLW time series.} \\
    % \multicolumn{2}{l}{$^b$ Equilibrium temperature calculations assume zero albedo and perfect heat redistribution.} 
\end{tabular}
\end{table}


% %$\ln{P}$ [days] & $\mathcal{N}(\ln{0.768},0.5)$ & - \\
% $P$ [days] & $\mathcal{U}(-\inf,\inf)$ \\
% $T_{0}$ [BJD-2,457,000] & $\mathcal{U}(-\inf,\inf)$  \\
% $\ln{r_p}$ [\Rearth{]} & $\mathcal{N}(0.5\cdot \ln(Z) + \ln{R_s},1)$\tablenotemark{b} \\
% $r_{p}/R_s$  & $\mathcal{U}(-\inf,\inf)$ \\
% $b$ & $\mathcal{U}(0,1+r_p/R_s)$ \\
% $\ln{K}$ [\mps{]} & $\mathcal{U}(-4,4)$ \\
% $e$ & $\mathcal{B}(0.867,3.03)$\tablenotemark{c} \\
% $\omega$ [rad] & $\mathcal{U}(-\pi,\pi)$\tablenotemark{c} \\
% $\sqrt{e}\cos{\omega}$ & $\mathcal{U}(-1,1)$ \\
% $\sqrt{e}\sin{\omega}$ & $\mathcal{U}(-1,1)$ \\

% \enddata
% \tablecomments{Gaussian distributions are denoted by $\mathcal{N}$ and are
%   parameterized by mean and standard deviation values. Uniform distributions
%   are denoted by $\mathcal{U}$ and bounded by the specified lower and upper
%   limits. Beta distributions are denoted by $\mathcal{B}$ and are parameterized
%   by the shape parameters $\alpha$ and $\beta$.}
% \tablenotetext{a}{$f'_{\rm PDCSAP}$ is the flux time series representing the dilution and background-corrected \texttt{PDCSAP} light curve from TESS.}
% \tablenotetext{b}{The transit depth of TOI-1634.01 reported by the SPOC: $Z=1520$ ppm.}
% \tablenotetext{c}{For use in the TESS analysis only \citealt{kipping13}.}
% \end{deluxetable}

==> results_fiducial.tex <==
\startlongtable
\begin{deluxetable*}{lcc}
\tabletypesize{\footnotesize}
\tablecaption{Point estimates of the TOI-1266 planetary system model parameters\label{tab:results}}
\tablewidth{0pt}
\tablehead{Parameter & Fiducial Model Values\tablenotemark{a} & \texttt{EXOFASTv2} Model Values\tablenotemark{b}}
\startdata
\multicolumn{3}{c}{\emph{TESS light curve parameters}} \\
$\ln{\omega_0}$ & $1.64\pm 1.15$ & - \\
$\ln{S_0 \omega_0^4}$ & $3.62^{+0.40}_{-0.39}$ & - \\
$\ln{s_{\text{TESS}}^2}$ & $1.21\pm 0.01$ & - \\
\tess{} limb darkening coefficient, $u_1$ & $0.28^{+0.33}_{-0.20}$ & $0.30^{+0.07}_{-0.05}$ \\
\tess{} limb darkening coefficient, $u_2$ & $0.16^{+0.37}_{-0.28}$ & $0.32^{+0.07}_{-0.06}$ \\
Dilution & - & $0.023^{+0.047}_{-0.048}$ \\
\smallskip \\

\multicolumn{3}{c}{\emph{RV parameters}} \\
$\Sigma_{rot}$ [\mps{]} & $1.42^{+0.34}_{-0.32}$ & - \\
$P_{\text{rot}}$ [days] & $32.09^{+0.49}_{-0.79}$ & - \\
$\ln{Q_0}$ & $0.74^{+0.79}_{-0.82}$ & - \\
$\ln{dQ}$ & $1.22^{+2.15}_{-2.76}$ & - \\
$f$ & $0.50^{+0.29}_{-0.29}$ & - \\
Jitter, $s$ [\mps{]} & $0.50^{+0.57}_{-0.39}$ & - \\
Systemic velocity, $\gamma$ [\mps{]} & $-40901.93533847075^{+0.26}_{-0.25}$ & - \\
\smallskip \\

\multicolumn{3}{c}{\emph{TOI-1266 b parameters}} \\
Orbital period, $P_b$ [days] & $10.89484\pm 0.000012$ &  - \\
Time of mid-transit, $T_{0,b}$ [BJD - 2,457,000] & $2649.7513\pm 0.0012$ & - \\
Transit duration $D_b$ [hrs] & $2.071^{+0.039}_{-0.032}$ & - \\
Transit depth, $Z_b$ [ppt] & $3.09^{+0.14}_{-0.14}$ & - \\
Scaled semimajor axis, $a_b/R_\star$ & $36.21^{+1.26}_{-1.21}$ & - \\
Planet-to-star radius ratio, $R_{p,b}/R_\star$ & $0.0556^{+0.0013}_{-0.0013}$ & - \\
Impact parameter, $b_b$ & $0.549^{+0.047}_{-0.057}$ & - \\
Inclination, $i_b$ [deg] & $89.13^{+0.11}_{-0.10}$ & - \\
Eccentricity, $e_b$ & $<0.20^a$ & - \\
Planet radius, $R_{p,b}$ [\Rearth{]} & $2.62^{+0.11}_{-0.11}$ & - \\
Log RV semi-amplitude, $\ln{K_b}$ & $0.70^{+0.16}_{-0.19}$ & - \\
RV semi-amplitude, $K_b$ [\mps{]} & $2.02^{+0.35}_{-0.35}$ & - \\
Planet mass, $M_{p,b}$ [\Mearth{]} & $3.93^{+0.71}_{-0.69}$ & - \\
Bulk density, $\rho_b$ [g cm$^{-3}$] & $1.21\pm 0.3$ & - \\
Surface gravity, $g_b$ [m s$^{-2}$] & $5.60\pm 1.1$ & - \\
Escape velocity, $v_{\text{esc},b}$ [km s$^{-1}$] & $13.8^{+1.2}_{-1.3}$ & - \\
Semimajor axis, $a_b$ [au] & $0.0728^{+0.0011}_{-0.0011}$ & - \\
Insolation, $F_b$ [F$_{\oplus}$] & $5.4^{+1.1}_{-0.9}$ & - \\
Equilibrium temperature$^b$, $T_{\text{eq},b}$ [K] & $425^{+20}_{-19}$ & - \\
\smallskip \\

\multicolumn{3}{c}{\emph{TOI-1266 c parameters}} \\
Orbital period, $P_c$ [days] & $18.801611\pm 0.000052$ & - \\
Time of mid-transit, $T_{0,c}$ [BJD - 2,457,000] & $2630.04642\pm 0.0025$ & - \\
Transit duration $D_c$ [hrs] & $1.951^{+0.081}_{-0.074}$ & - \\
Transit depth, $Z_c$ [ppt] & $2.05^{+0.18}_{-0.17}$ & - \\
Scaled semimajor axis, $a_c/R_\star$ & $52.10^{+1.82}_{-1.74}$ & - \\
Planet-to-star radius ratio, $R_{p,c}/R_\star$ & $0.0453^{+0.0020}_{-0.0019}$ &  - \\
Impact parameter, $b_c$ & $0.769^{+0.030}_{-0.035}$ & - \\
Inclination, $i_c$ [deg] & $89.15^{+0.06}_{-0.06}$ & - \\

$e_c\cos{\omega_c}$ & - & $-0.05^{+0.07}_{-0.08}$ \\
$e_c\sin{\omega_c}$ & - & $0.15^{+0.15}_{-0.13}$ \\
$\sqrt{e_c}\cos{\omega_c}$ & $0.13^{+0.12}_{-0.15}$ & - \\
$\sqrt{e_c}\sin{\omega_c}$ & $0.07^{+0.17}_{-0.19}$ & - \\
Eccentricity, $e_c$ & $<0.41^a$ & - \\
Argument of periastron, $\omega_c$ [deg] & $124^{+87}_{-147}$ & $111^{+39}_{-27}$ \\

Planet radius, $R_{p,c}$ [\Rearth{]} & $2.13^{+0.12}_{-0.12}$ & - \\
Log RV semi-amplitude, $\ln{K_c}$ & $0.34^{+0.24}_{-0.32}$ & - \\
RV semi-amplitude, $K_c$ [\mps{]} & $1.40^{+0.38}_{-0.38}$ & - \\
Planet mass, $M_{p,c}$ [\Mearth{]} & $3.28^{+0.90}_{-0.89}$ & - \\
Bulk density, $\rho_c$ [g cm$^{-3}$] & $1.8^{+0.7}_{-0.6}$ & - \\
Surface gravity, $g_c$ [m s$^{-2}$] & $7.0^{+2.2}_{-2.0}$ & - \\
Escape velocity, $v_{\text{esc},c}$ [km s$^{-1}$] & $13.8^{+1.2}_{-1.3}$ & - \\
Semimajor axis, $a_c$ [au] & $0.1047^{+0.0016}_{-0.0016}$ & - \\
Insolation, $F_c$ [F$_{\oplus}$] & $2.6^{+0.5}_{-0.4}$ & - \\
Equilibrium temperature$^b$, $T_{\text{eq},c}$ [K] & $354^{+17}_{-16}$ & \\
\enddata
\tablenotetext{a}{95\% upper limit.}
\tablenotetext{b}{Equilibrium temperature calculations assume zero albedo and perfect heat redistribution.}
%\tablecomments{}
\end{deluxetable*}


==> rvs_orig.tex <==
\newpage
\begin{landscape}
\begin{table*}
\centering
\label{tab:rv}
\begin{tabular}{rrrrrrrrrrrrrrr}
\toprule
Time & LBL RV & $\sigma_{RV}$ & $B$-band & $\sigma_{B,RV}$ & $V$-band & $\sigma_{V,RV}$ & $R$-band & $\sigma_{R,RV}$ & LBL DLW & $\sigma_{DLW}$ & FWHM & $\sigma_{FWHM}$ & BIS & $\sigma_{BIS}$ \\ 
$[$BJD - 2,457,000$]$ & [m/s] & [m/s] & RV [m/s] & [m/s] & RV [m/s] & [m/s] & RV [m/s] & [m/s] & [m$^2$/s$^2$] & [m$^2$/s$^2$] & [km/s] & [km/s] & [km/s] & [km/s] \\
\midrule
 1977.51159 &    -40901.22 &            1.84 &  -40899.08 &          5.70 &  -40897.83 &          3.12 &  -40905.35 &          2.61 &        17004.81 &            1703.61 &        4.33 &           0.01 &       0.04 &          0.01 \\
 1978.51986 &    -40905.47 &            1.88 &  -40916.26 &          6.03 &  -40899.37 &          3.26 &  -40907.08 &          2.60 &        19303.85 &            1752.88 &        4.35 &           0.01 &       0.04 &          0.01 \\
 1979.53014 &    -40896.99 &            2.18 &  -40882.53 &          8.75 &  -40898.41 &          4.17 &  -40898.41 &          2.73 &         8964.15 &            2102.83 &        4.34 &           0.01 &       0.04 &          0.01 \\
 % 1983.53921 &    -40900.62 &            4.51 &  -40923.18 &         16.07 &  -40877.26 &          8.90 &  -40905.46 &          5.61 &         3474.90 &            4138.46 &        4.35 &           0.03 &       0.01 &          0.03 \\
 % 1985.48122 &    -40899.25 &            2.22 &  -40889.92 &          9.35 &  -40890.89 &          4.32 &  -40904.21 &          2.75 &           22.65 &            2161.65 &        3.27 &           0.01 &       0.00 &          0.01 \\
 % 1986.45249 &    -40901.72 &            1.64 &  -40897.54 &          5.61 &  -40900.37 &          2.92 &  -40902.68 &          2.19 &        16148.33 &            1554.74 &        3.27 &           0.01 &       0.00 &          0.01 \\
 % 1987.42286 &    -40900.57 &            2.44 &  -40897.10 &          9.47 &  -40901.19 &          4.54 &  -40901.21 &          3.09 &         3921.15 &            2335.44 &        3.28 &           0.01 &       0.01 &          0.01 \\
 % 1988.50707 &    -40899.57 &            2.42 &  -40893.41 &         10.84 &  -40896.59 &          4.93 &  -40901.84 &          2.91 &        -1232.86 &            2371.15 &        3.29 &           0.01 &      -0.00 &          0.01 \\
 % 1989.50729 &    -40905.81 &            2.74 &  -40874.94 &          9.92 &  -40907.31 &          4.99 &  -40907.86 &          3.57 &         4263.25 &            2596.92 &        3.28 &           0.01 &       0.01 &          0.01 \\
 % 1990.53022 &    -40896.98 &            2.35 &  -40888.60 &          7.10 &  -40897.46 &          3.91 &  -40897.54 &          3.42 &        13168.29 &            2170.31 &        3.27 &           0.01 &       0.00 &          0.01 \\
 % 1993.46312 &    -40895.49 &            4.06 &  -40892.09 &         12.26 &  -40894.25 &          7.16 &  -40894.25 &          5.61 &        12489.57 &            3637.54 &        3.27 &           0.02 &       0.01 &          0.02 \\
 % 2007.43414 &    -40900.00 &            1.56 &  -40893.76 &          4.36 &  -40899.67 &          2.57 &  -40902.40 &          2.35 &        23622.26 &            1421.18 &        3.27 &           0.00 &       0.00 &          0.00 \\
 % 2008.45874 &    -40900.41 &            1.77 &  -40898.63 &          5.34 &  -40899.35 &          2.98 &  -40900.92 &          2.58 &        18831.99 &            1639.07 &        3.27 &           0.01 &       0.01 &          0.01 \\
 % 2019.43293 &    -40900.40 &            1.96 &  -40900.78 &          6.33 &  -40898.56 &          3.36 &  -40901.64 &          2.73 &        18676.30 &            1839.29 &        3.28 &           0.01 &       0.00 &          0.01 \\
 % 2026.41807 &    -40902.12 &            2.40 &  -40905.11 &          7.82 &  -40897.83 &          4.13 &  -40903.69 &          3.31 &        12962.71 &            2248.88 &        3.29 &           0.01 &       0.00 &          0.01 \\
 % 2027.41749 &    -40899.77 &            2.02 &  -40899.66 &          5.12 &  -40898.24 &          3.17 &  -40899.85 &          3.39 &        24954.89 &            1795.16 &        3.28 &           0.01 &      -0.00 &          0.01 \\
 % 2028.46370 &    -40902.05 &            1.91 &  -40895.74 &          6.30 &  -40902.68 &          3.32 &  -40902.17 &          2.63 &        18306.80 &            1800.47 &        3.28 &           0.01 &       0.00 &          0.01 \\
 % 2235.74255 &    -40899.71 &            2.18 &  -40897.16 &          7.56 &  -40895.13 &          3.80 &  -40903.96 &          2.95 &         3688.45 &            2064.58 &        3.27 &           0.01 &       0.00 &          0.01 \\
 % 2236.70230 &    -40904.72 &            2.29 &  -40904.54 &          8.14 &  -40900.40 &          4.01 &  -40908.11 &          3.06 &         1792.02 &            2169.93 &        3.26 &           0.01 &       0.00 &          0.01 \\
 % 2237.78136 &    -40906.81 &            3.19 &  -40928.51 &         19.70 &  -40907.03 &          6.12 &  -40905.53 &          3.78 &       -13324.17 &            3161.35 &        2.99 &           0.01 &       0.40 &          0.01 \\
 % 2239.73602 &    -40900.15 &            1.73 &  -40897.82 &          5.81 &  -40896.02 &          3.00 &  -40904.63 &          2.37 &        11691.92 &            1637.85 &        3.27 &           0.01 &       0.01 &          0.01 \\
 % 2240.76401 &    -40899.59 &            1.73 &  -40890.90 &          6.26 &  -40901.69 &          3.11 &  -40900.46 &          2.29 &         8265.69 &            1658.21 &        3.27 &           0.01 &       0.01 &          0.01 \\
 % 2244.69650 &    -40899.42 &            1.75 &  -40897.58 &          5.83 &  -40899.70 &          3.02 &  -40899.67 &          2.41 &        12698.43 &            1652.51 &        3.26 &           0.01 &       0.00 &          0.01 \\
 % 2246.73306 &    -40898.12 &            3.95 &  -40862.72 &         13.50 &  -40901.51 &          7.14 &  -40899.43 &          5.21 &          782.09 &            3629.26 &        3.25 &           0.02 &       0.00 &          0.02 \\
 % 2253.78600 &    -40904.17 &            1.77 &  -40899.72 &          5.49 &  -40902.83 &          2.96 &  -40907.09 &          2.56 &        12321.65 &            1656.89 &        3.26 &           0.01 &       0.00 &          0.01 \\
 % 2255.74340 &    -40907.50 &            2.34 &  -40903.21 &         10.19 &  -40897.44 &          4.49 &  -40912.57 &          2.89 &        -6124.73 &            2284.84 &        3.27 &           0.01 &      -0.00 &          0.01 \\
 % 2256.75052 &    -40900.40 &            2.41 &  -40888.75 &          8.20 &  -40896.19 &          4.14 &  -40907.98 &          3.31 &         1018.24 &            2274.02 &        3.25 &           0.01 &       0.01 &          0.01 \\
 % 2272.62641 &    -40901.90 &            2.00 &  -40906.74 &          7.06 &  -40901.12 &          3.51 &  -40902.14 &          2.68 &         8539.97 &            1905.53 &        3.25 &           0.01 &      -0.00 &          0.01 \\
 % 2275.61611 &    -40902.18 &            2.12 &  -40897.35 &          6.58 &  -40898.45 &          3.56 &  -40908.26 &          3.06 &        10867.90 &            1977.35 &        3.27 &           0.01 &       0.00 &          0.01 \\
 % 2276.66086 &    -40897.69 &            2.03 &  -40897.13 &          6.36 &  -40897.65 &          3.42 &  -40898.69 &          2.90 &        10039.11 &            1904.12 &        3.27 &           0.01 &       0.00 &          0.01 \\
 % 2277.69495 &    -40897.49 &            1.90 &  -40894.96 &          6.22 &  -40899.09 &          3.26 &  -40897.38 &          2.64 &        11262.72 &            1781.94 &        3.27 &           0.01 &       0.00 &          0.01 \\
 % 2288.70515 &    -40899.32 &            1.89 &  -40900.84 &          7.27 &  -40889.24 &          3.49 &  -40903.17 &          2.42 &         6810.12 &            1828.73 &        3.27 &           0.01 &       0.01 &          0.01 \\
 % 2289.60849 &    -40904.16 &            1.78 &  -40902.98 &          6.08 &  -40900.43 &          3.15 &  -40905.85 &          2.41 &        10525.00 &            1695.94 &        3.27 &           0.01 &       0.00 &          0.01 \\
 % 2298.51394 &    -40900.36 &            4.13 &  -40893.58 &         14.62 &  -40896.69 &          7.74 &  -40901.95 &          5.30 &        -8152.67 &            3791.96 &        3.23 &           0.02 &      -0.01 &          0.02 \\
 % 2299.70626 &    -40901.70 &            2.88 &  -40897.81 &         11.84 &  -40898.91 &          5.48 &  -40903.49 &          3.59 &        -2774.57 &            2774.92 &        3.26 &           0.01 &       0.01 &          0.01 \\
 % 2304.63253 &    -40890.48 &            3.90 &  -40883.38 &         14.68 &  -40887.12 &          7.57 &  -40892.84 &          4.86 &         1506.28 &            3640.56 &        3.26 &           0.02 &       0.02 &          0.02 \\
 % 2306.56900 &    -40901.92 &            5.00 &  -40882.32 &         16.47 &  -40901.23 &          9.76 &  -40907.23 &          6.30 &         7624.36 &            4438.66 &        3.19 &           0.02 &      -0.00 &          0.02 \\
 % 2307.54068 &    -40899.80 &            1.87 &  -40888.09 &          9.35 &  -40895.18 &          3.89 &  -40902.43 &          2.20 &         1183.08 &            1865.34 &        3.27 &           0.01 &       0.00 &          0.01 \\
 % 2323.62312 &    -40907.90 &            2.58 &  -40894.72 &          9.05 &  -40897.73 &          4.54 &  -40914.63 &          3.47 &         4236.89 &            2434.45 &        3.26 &           0.01 &      -0.00 &          0.01 \\
 % 2326.55520 &    -40903.53 &            2.12 &  -40896.96 &          5.82 &  -40901.44 &          3.38 &  -40909.16 &          3.32 &        20048.41 &            1919.86 &        3.26 &           0.01 &       0.01 &          0.01 \\
 % 2327.50579 &    -40903.23 &            1.67 &  -40884.27 &          6.12 &  -40900.92 &          3.00 &  -40906.50 &          2.19 &        12689.12 &            1605.27 &        3.28 &           0.01 &       0.01 &          0.01 \\
 % 2328.55859 &    -40901.21 &            2.91 &  -40893.69 &         12.93 &  -40894.65 &          5.95 &  -40903.36 &          3.49 &        -4168.75 &            2830.72 &        3.27 &           0.01 &       0.00 &          0.01 \\
 % 2330.66652 &    -40901.35 &            2.18 &  -40910.35 &          9.76 &  -40895.58 &          4.26 &  -40904.28 &          2.66 &         5723.78 &            2140.54 &        3.25 &           0.01 &       0.01 &          0.01 \\
 % 2332.64729 &    -40904.95 &            2.45 &  -40908.54 &         10.54 &  -40900.37 &          4.79 &  -40906.79 &          3.02 &         -421.09 &            2389.32 &        3.25 &           0.01 &      -0.00 &          0.01 \\
 % 2333.66758 &    -40901.62 &            2.21 &  -40908.90 &          9.33 &  -40890.43 &          4.20 &  -40904.98 &          2.75 &         2209.36 &            2151.46 &        3.25 &           0.01 &       0.01 &          0.01 \\
 % 2343.59452 &    -40894.65 &            2.73 &  -40911.74 &         13.92 &  -40884.65 &          6.01 &  -40896.82 &          3.16 &        -9784.66 &            2701.29 &        3.27 &           0.02 &      -0.00 &          0.02 \\
 % 2344.63199 &    -40895.97 &            2.86 &  -40904.75 &         15.45 &  -40878.94 &          7.03 &  -40898.57 &          3.21 &        -6032.13 &            2841.28 &        2.94 &           0.01 &       0.47 &          0.01 \\
 % 2345.49714 &    -40897.17 &            2.48 &  -40889.31 &         13.76 &  -40890.63 &          5.81 &  -40899.51 &          2.81 &        -8313.03 &            2482.14 &        2.95 &           0.01 &      -0.46 &          0.01 \\
 % 2360.54044 &    -40900.23 &            2.66 &  -40886.92 &         12.18 &  -40886.49 &          5.35 &  -40906.38 &          3.21 &         -660.15 &            2607.67 &        3.26 &           0.01 &       0.01 &          0.01 \\
 % 2363.54156 &    -40899.72 &            1.98 &  -40891.69 &          7.45 &  -40894.93 &          3.57 &  -40903.63 &          2.58 &         7302.46 &            1902.44 &        3.26 &           0.01 &       0.00 &          0.01 \\
 % 2364.53741 &    -40898.25 &            2.10 &  -40897.52 &          7.32 &  -40896.45 &          3.64 &  -40898.28 &          2.84 &        11941.03 &            1987.66 &        3.26 &           0.01 &       0.01 &          0.01 \\
 % 2365.52246 &    -40898.48 &            2.40 &  -40892.32 &          9.40 &  -40897.16 &          4.44 &  -40902.29 &          3.06 &         1128.14 &            2304.87 &        3.26 &           0.01 &       0.00 &          0.01 \\
 % 2366.53863 &    -40903.88 &            1.70 &  -40891.23 &          6.07 &  -40902.95 &          3.03 &  -40905.38 &          2.25 &        12292.02 &            1620.31 &        3.26 &           0.01 &       0.00 &          0.01 \\
 % 2367.50570 &    -40904.84 &            1.61 &  -40905.87 &          5.04 &  -40902.64 &          2.73 &  -40906.98 &          2.30 &        18511.37 &            1506.84 &        3.26 &           0.01 &       0.00 &          0.01 \\
 % 2377.47566 &    -40902.42 &            2.39 &  -40910.35 &          8.99 &  -40901.29 &          4.28 &  -40901.78 &          3.13 &         2352.20 &            2277.05 &        3.27 &           0.01 &       0.01 &          0.01 \\
 % 2378.44354 &    -40902.96 &            2.02 &  -40903.70 &          7.86 &  -40899.17 &          3.71 &  -40905.30 &          2.60 &         5198.87 &            1957.67 &        3.26 &           0.01 &       0.01 &          0.01 \\
 % 2379.44686 &    -40901.02 &            2.32 &  -40912.13 &          8.55 &  -40895.93 &          4.13 &  -40903.11 &          3.07 &         7834.88 &            2213.54 &        3.29 &           0.01 &       0.01 &          0.01 \\
 % 2387.40960 &    -40905.28 &            2.02 &  -40900.77 &          6.77 &  -40907.41 &          3.48 &  -40904.29 &          2.79 &        10404.88 &            1907.40 &        3.27 &           0.01 &       0.00 &          0.01 \\
 % 2388.43950 &    -40901.86 &            1.68 &  -40902.57 &          5.84 &  -40901.48 &          2.93 &  -40901.56 &          2.29 &        10148.82 &            1602.45 &        3.26 &           0.01 &       0.01 &          0.01 \\
 % 2390.43065 &    -40914.02 &            2.00 &  -40920.70 &          7.11 &  -40911.08 &          3.50 &  -40914.10 &          2.68 &        10763.08 &            1905.37 &        3.25 &           0.01 &       0.00 &          0.01 \\
 % 2391.44130 &    -40904.60 &            2.34 &  -40914.38 &          8.60 &  -40905.88 &          4.17 &  -40903.29 &          3.10 &         7978.99 &            2240.76 &        3.25 &           0.01 &       0.01 &          0.01 \\
 % 2392.42735 &    -40901.00 &            1.73 &  -40894.88 &          5.82 &  -40900.05 &          3.01 &  -40903.10 &          2.37 &        11038.03 &            1643.07 &        3.27 &           0.01 &       0.01 &          0.01 \\
 % 2414.37483 &    -40902.55 &            2.14 &  -40900.37 &          8.28 &  -40902.40 &          3.79 &  -40903.10 &          2.82 &         7164.02 &            2070.51 &        3.24 &           0.01 &       0.01 &          0.01 \\
 % 2415.40471 &    -40899.35 &            2.15 &  -40898.46 &          7.69 &  -40900.29 &          3.78 &  -40899.89 &          2.89 &         5051.41 &            2056.47 &        3.26 &           0.01 &       0.01 &          0.01 \\
 % 2416.38125 &    -40900.75 &            1.54 &  -40892.26 &          4.86 &  -40898.23 &          2.61 &  -40902.39 &          2.18 &        17524.64 &            1442.50 &        3.27 &           0.01 &      -0.00 &          0.01 \\
 % 2566.76980 &    -40901.19 &            2.30 &  -40893.29 &          7.93 &  -40899.50 &          3.81 &  -40902.41 &          3.24 &        -5246.07 &            2178.45 &        3.24 &           0.01 &       0.01 &          0.01 \\
 % 2579.78023 &    -40904.88 &            2.08 &  -40892.34 &          6.74 &  -40906.23 &          3.39 &  -40906.30 &          3.03 &         3785.31 &            1961.06 &        3.25 &           0.01 &       0.01 &          0.01 \\
 % 2580.77244 &    -40893.70 &            3.75 &  -40883.52 &         11.56 &  -40887.82 &          6.00 &  -40894.52 &          5.58 &       -14218.38 &            3400.59 &        3.25 &           0.02 &       0.03 &          0.02 \\
 % 2581.80652 &    -40902.26 &            2.04 &  -40895.56 &          6.55 &  -40907.85 &          3.27 &  -40901.13 &          3.00 &         4952.66 &            1914.06 &        3.24 &           0.01 &       0.00 &          0.01 \\
 % 2582.78153 &    -40897.12 &            4.52 &  -40874.64 &         15.04 &  -40901.76 &          7.91 &  -40894.26 &          6.09 &       -17150.01 &            4106.68 &        3.24 &           0.02 &       0.01 &          0.02 \\
 % 2583.75768 &    -40901.94 &            1.83 &  -40890.99 &          5.92 &  -40903.24 &          3.03 &  -40903.34 &          2.64 &         4449.59 &            1733.63 &        3.25 &           0.01 &       0.00 &          0.01 \\
 % 2601.75253 &    -40895.99 &            1.95 &  -40887.54 &          7.10 &  -40896.18 &          3.36 &  -40897.80 &          2.64 &          235.90 &            1874.99 &        3.25 &           0.01 &       0.01 &          0.01 \\
 % 2614.76472 &    -40903.14 &            3.24 &  -40896.16 &          9.63 &  -40902.26 &          5.11 &  -40905.43 &          4.98 &         -452.21 &            2959.02 &        3.28 &           0.01 &       0.00 &          0.01 \\
 % 2615.77606 &    -40901.22 &            2.36 &  -40889.80 &          7.06 &  -40903.80 &          3.73 &  -40900.44 &          3.65 &         5057.56 &            2190.08 &        3.27 &           0.01 &       0.01 &          0.01 \\
 % 2625.70022 &    -40900.80 &            2.05 &  -40884.88 &          6.21 &  -40902.67 &          3.26 &  -40904.11 &          3.12 &         7572.34 &            1911.81 &        3.26 &           0.01 &       0.01 &          0.01 \\
 % 2627.70728 &    -40899.60 &            2.39 &  -40898.97 &          7.93 &  -40901.74 &          3.89 &  -40897.63 &          3.45 &         1183.82 &            2247.72 &        3.25 &           0.01 &       0.01 &          0.01 \\
 % 2642.70256 &    -40900.67 &            2.38 &  -40894.63 &          8.32 &  -40902.88 &          4.00 &  -40899.94 &          3.30 &          994.85 &            2267.78 &        3.27 &           0.01 &      -0.00 &          0.01 \\
 % 2648.66780 &    -40904.59 &            2.46 &  -40902.88 &          9.44 &  -40901.98 &          4.35 &  -40907.66 &          3.23 &        -3768.02 &            2378.44 &        3.27 &           0.01 &       0.01 &          0.01 \\
 % 2649.56725 &    -40905.76 &            2.02 &  -40904.25 &          6.40 &  -40909.53 &          3.29 &  -40905.22 &          2.95 &         7698.65 &            1905.98 &        3.27 &           0.01 &       0.00 &          0.01 \\
 % 2651.67282 &    -40908.47 &            1.58 &  -40898.52 &          5.09 &  -40907.80 &          2.64 &  -40911.68 &          2.26 &        11687.43 &            1493.37 &        3.26 &           0.01 &       0.00 &          0.01 \\
 % 2659.66560 &    -40898.28 &            1.78 &  -40902.77 &          5.25 &  -40897.69 &          2.87 &  -40895.50 &          2.72 &         9404.64 &            1651.16 &        3.26 &           0.01 &       0.00 &          0.01 \\
 % 2682.54112 &    -40899.08 &            1.79 &  -40902.55 &          5.65 &  -40899.91 &          2.93 &  -40897.64 &          2.60 &        11041.35 &            1682.59 &        3.27 &           0.01 &       0.01 &          0.01 \\
 % 2686.57001 &    -40901.15 &            4.02 &  -40907.31 &         14.05 &  -40907.03 &          7.08 &  -40896.90 &          5.36 &         5003.62 &            3728.31 &        3.25 &           0.02 &       0.01 &          0.02 \\
 % 2690.64626 &    -40899.51 &            2.59 &  -40895.86 &         11.40 &  -40896.91 &          4.93 &  -40901.11 &          3.21 &        -6781.32 &            2529.60 &        3.24 &           0.01 &       0.01 &          0.01 \\
 % 2705.61485 &    -40906.07 &            2.16 &  -40912.78 &          7.86 &  -40903.25 &          3.71 &  -40906.42 &          2.94 &        -4063.61 &            2081.30 &        3.25 &           0.01 &      -0.01 &          0.01 \\
 % 2706.55841 &    -40906.14 &            2.15 &  -40903.30 &          6.80 &  -40904.96 &          3.48 &  -40907.21 &          3.18 &         5092.49 &            2026.15 &        3.25 &           0.01 &       0.01 &          0.01 \\
 % 2707.54897 &    -40908.13 &            2.13 &  -40924.13 &          7.36 &  -40904.76 &          3.62 &  -40907.46 &          2.93 &         4926.22 &            2033.84 &        3.26 &           0.01 &       0.01 &          0.01 \\
 % 2708.50376 &    -40912.11 &            3.19 &  -40912.86 &         11.47 &  -40914.01 &          5.56 &  -40911.03 &          4.29 &        -9255.96 &            3021.42 &        3.28 &           0.01 &      -0.01 &          0.01 \\
 % 2709.43856 &    -40902.15 &            2.70 &  -40901.33 &          9.75 &  -40898.92 &          4.68 &  -40904.86 &          3.63 &        -3626.35 &            2572.81 &        3.26 &           0.01 &      -0.00 &          0.01 \\
 % 2712.53794 &    -40906.58 &            2.90 &  -40896.21 &         10.78 &  -40914.01 &          5.08 &  -40905.31 &          3.86 &         -315.43 &            2760.16 &        3.26 &           0.01 &       0.02 &          0.01 \\
 % 2714.56851 &    -40903.09 &            1.80 &  -40901.60 &          6.05 &  -40903.30 &          3.03 &  -40904.30 &          2.53 &        11560.08 &            1707.72 &        3.25 &           0.01 &       0.01 &          0.01 \\
 % 2715.54425 &    -40901.89 &            2.36 &  -40902.78 &          7.22 &  -40902.50 &          3.79 &  -40903.69 &          3.54 &         8444.52 &            2182.56 &        3.26 &           0.01 &       0.00 &          0.01 \\
 % 2716.53446 &    -40905.39 &            1.82 &  -40894.51 &          6.51 &  -40906.63 &          3.14 &  -40906.21 &          2.47 &         6337.37 &            1738.65 &        3.26 &           0.01 &       0.01 &          0.01 \\
 % 2717.52028 &    -40904.28 &            1.46 &  -40897.02 &          4.46 &  -40904.38 &          2.44 &  -40905.26 &          2.12 &        14663.39 &            1365.41 &        3.26 &           0.00 &       0.00 &          0.00 \\
 % 2718.49378 &    -40901.90 &            1.53 &  -40895.09 &          4.98 &  -40903.61 &          2.62 &  -40900.44 &          2.15 &        12954.57 &            1443.81 &        3.26 &           0.01 &       0.01 &          0.01 \\
 % 2735.51101 &    -40898.78 &            2.34 &  -40883.40 &          9.64 &  -40901.09 &          4.31 &  -40899.37 &          2.98 &         -988.05 &            2283.88 &        3.26 &           0.01 &       0.01 &          0.01 \\
 % 2737.39915 &    -40905.63 &            4.30 &  -40897.25 &         14.53 &  -40917.84 &          7.55 &  -40901.90 &          5.80 &        -2717.31 &            3921.61 &        3.26 &           0.02 &       0.02 &          0.02 \\
 % 2738.46524 &    -40906.47 &            2.92 &  -40907.06 &          9.01 &  -40913.95 &          4.74 &  -40901.20 &          4.31 &         1120.68 &            2678.43 &        3.27 &           0.01 &      -0.01 &          0.01 \\
 % 2739.52841 &    -40907.27 &            2.53 &  -40915.69 &          9.44 &  -40906.59 &          4.41 &  -40907.55 &          3.39 &         5269.96 &            2413.81 &        3.27 &           0.01 &      -0.01 &          0.01 \\
 % 2747.46584 &    -40902.68 &            1.89 &  -40901.21 &          7.03 &  -40903.60 &          3.32 &  -40901.87 &          2.52 &         7917.06 &            1815.88 &        3.26 &           0.01 &       0.01 &          0.01 \\
 % 2748.48771 &    -40908.10 &            2.77 &  -40917.33 &         10.60 &  -40905.81 &          4.93 &  -40907.21 &          3.62 &         1506.55 &            2642.70 &        3.26 &           0.01 &       0.01 &          0.01 \\
 % 2750.43470 &    -40902.14 &            2.74 &  -40902.46 &         10.10 &  -40896.21 &          4.76 &  -40906.82 &          3.67 &         3251.64 &            2603.95 &        3.27 &           0.01 &       0.01 &          0.01 \\
 % 2751.46868 &    -40905.67 &            1.65 &  -40902.81 &          5.77 &  -40908.08 &          2.86 &  -40906.13 &          2.26 &         9878.33 &            1580.69 &        3.26 &           0.01 &       0.01 &          0.01 \\
 % 2752.48380 &    -40901.55 &            2.04 &  -40899.92 &          6.90 &  -40900.26 &          3.44 &  -40902.15 &          2.86 &        10412.17 &            1938.02 &        3.28 &           0.01 &      -0.01 &          0.01 \\
 % 2760.38433 &    -40896.67 &            2.73 &  -40880.52 &          9.35 &  -40899.42 &          4.60 &  -40895.73 &          3.81 &         2215.12 &            2577.01 &        3.23 &           0.01 &       0.01 &          0.01 \\
 % 2768.42522 &    -40901.27 &            2.26 &  -40894.24 &          7.70 &  -40902.31 &          3.83 &  -40901.55 &          3.14 &         3094.78 &            2140.29 &        3.27 &           0.01 &       0.00 &          0.01 \\
 % 2769.40911 &    -40902.35 &            3.29 &  -40899.21 &         11.94 &  -40901.19 &          5.73 &  -40903.48 &          4.40 &        -3479.22 &            3098.82 &        3.26 &           0.02 &       0.00 &          0.02 \\
 % 2772.40655 &    -40902.75 &            1.55 &  -40889.25 &          5.01 &  -40901.23 &          2.62 &  -40904.91 &          2.21 &        10514.58 &            1463.51 &        3.26 &           0.01 &       0.01 &          0.01 \\
 % 2773.39372 &    -40905.64 &            1.52 &  -40908.84 &          4.79 &  -40905.43 &          2.55 &  -40905.94 &          2.20 &        14224.99 &            1430.29 &        3.27 &           0.01 &       0.01 &          0.01 \\
 % 2774.41535 &    -40901.85 &            1.72 &  -40903.92 &          5.25 &  -40903.24 &          2.80 &  -40899.88 &          2.57 &        11630.19 &            1612.04 &        3.26 &           0.01 &       0.01 &          0.01 \\
 % 2775.38815 &    -40901.95 &            2.85 &  -40908.26 &          9.46 &  -40899.96 &          4.74 &  -40901.58 &          4.03 &        -1511.16 &            2678.46 &        3.27 &           0.01 &       0.00 &          0.01 \\
 % 2931.79415 &    -40903.19 &            2.49 &  -40904.56 &          8.39 &  -40905.07 &          4.11 &  -40899.91 &          3.56 &         1690.83 &            2342.20 &        3.27 &           0.01 &       0.01 &          0.01 \\
 % 2932.79227 &    -40906.31 &            2.75 &  -40896.79 &          8.06 &  -40908.91 &          4.35 &  -40905.88 &          4.32 &         3052.89 &            2524.18 &        3.28 &           0.01 &       0.00 &          0.01 \\
 % 2933.78002 &    -40907.83 &            2.28 &  -40901.40 &          7.18 &  -40910.86 &          3.71 &  -40905.21 &          3.35 &          696.40 &            2133.07 &        3.27 &           0.01 &       0.00 &          0.01 \\
 % 2934.79392 &    -40907.29 &            2.34 &  -40900.11 &          7.23 &  -40909.59 &          3.76 &  -40908.92 &          3.52 &         5657.49 &            2181.55 &        3.26 &           0.01 &       0.01 &          0.01 \\
 % 2937.75819 &    -40906.30 &            1.99 &  -40908.77 &          6.27 &  -40909.35 &          3.26 &  -40901.88 &          2.92 &         7120.31 &            1864.35 &        3.26 &           0.01 &       0.00 &          0.01 \\
 % 2959.72805 &    -40906.79 &            2.96 &  -40925.84 &         11.74 &  -40907.42 &          5.49 &  -40904.92 &          3.77 &        -7102.49 &            2839.69 &        3.27 &           0.01 &      -0.00 &          0.01 \\
 % 2962.74591 &    -40899.98 &            2.43 &  -40889.33 &          8.61 &  -40903.01 &          4.14 &  -40900.88 &          3.34 &        -1273.68 &            2314.28 &        3.28 &           0.01 &      -0.01 &          0.01 \\
 % 2963.75273 &    -40899.40 &            3.05 &  -40882.16 &         10.58 &  -40901.22 &          5.20 &  -40900.54 &          4.18 &        -6736.02 &            2872.06 &        3.26 &           0.01 &       0.00 &          0.01 \\
 % 2972.73000 &    -40902.16 &            2.60 &  -40907.46 &          8.73 &  -40901.33 &          4.37 &  -40904.65 &          3.65 &         -379.05 &            2447.78 &        3.27 &           0.01 &       0.01 &          0.01 \\
 % 2983.66649 &    -40896.39 &            2.44 &  -40887.54 &          9.28 &  -40892.04 &          4.31 &  -40900.29 &          3.23 &        -1355.75 &            2348.55 &        3.25 &           0.01 &      -0.00 &          0.01 \\
 % 3002.73614 &    -40903.87 &            2.55 &  -40907.29 &          7.59 &  -40906.30 &          4.03 &  -40901.33 &          3.92 &         5538.45 &            2336.79 &        3.27 &           0.01 &      -0.00 &          0.01 \\
 % 3004.67709 &    -40900.67 &            1.78 &  -40895.80 &          6.53 &  -40906.67 &          3.10 &  -40898.31 &          2.40 &         5243.91 &            1725.46 &        3.25 &           0.01 &      -0.01 &          0.01 \\
 % 3005.62174 &    -40900.43 &            1.86 &  -40900.30 &          5.62 &  -40900.16 &          3.00 &  -40899.55 &          2.80 &         7318.93 &            1733.41 &        3.26 &           0.01 &       0.01 &          0.01 \\
 % 3006.58584 &    -40901.64 &            2.46 &  -40891.70 &          7.96 &  -40904.02 &          3.98 &  -40899.12 &          3.60 &         5321.81 &            2297.61 &        3.27 &           0.01 &       0.01 &          0.01 \\
 % 3007.59296 &    -40905.31 &            2.09 &  -40901.93 &          6.58 &  -40904.75 &          3.39 &  -40907.95 &          3.06 &         5445.02 &            1965.91 &        3.27 &           0.01 &       0.00 &          0.01 \\
 % 3008.59780 &    -40904.43 &            2.83 &  -40918.98 &         10.69 &  -40900.44 &          5.00 &  -40904.03 &          3.73 &        -3988.41 &            2713.22 &        3.26 &           0.01 &       0.01 &          0.01 \\
 % 3009.65394 &    -40903.60 &            1.80 &  -40897.54 &          6.46 &  -40906.19 &          3.08 &  -40902.72 &          2.47 &         6249.28 &            1723.40 &        3.27 &           0.01 &       0.00 &          0.01 \\
 % 3010.60477 &    -40907.97 &            2.17 &  -40899.03 &          7.67 &  -40905.23 &          3.70 &  -40908.45 &          2.99 &         3150.99 &            2075.15 &        3.26 &           0.01 &       0.01 &          0.01 \\
 % 3011.58791 &    -40909.89 &            2.21 &  -40895.77 &          8.28 &  -40906.78 &          3.87 &  -40915.79 &          2.95 &         3339.53 &            2137.02 &        3.25 &           0.01 &       0.00 &          0.01 \\
 % 3012.61598 &    -40906.12 &            2.07 &  -40891.21 &          7.24 &  -40908.92 &          3.52 &  -40908.21 &          2.87 &         7673.23 &            1968.45 &        3.25 &           0.01 &      -0.01 &          0.01 \\
 % 3018.70124 &    -40901.81 &            2.16 &  -40907.45 &          6.28 &  -40900.24 &          3.38 &  -40903.49 &          3.42 &         8461.88 &            1988.61 &        3.26 &           0.01 &       0.01 &          0.01 \\
 % 3021.59658 &    -40900.32 &            3.29 &  -40897.27 &          9.97 &  -40904.51 &          5.28 &  -40897.54 &          4.96 &         1768.17 &            3008.74 &        3.27 &           0.01 &       0.01 &          0.01 \\
 % 3022.62535 &    -40904.21 &            2.43 &  -40899.56 &          9.28 &  -40906.40 &          4.28 &  -40905.11 &          3.21 &        -5364.95 &            2339.61 &        3.26 &           0.01 &       0.01 &          0.01 \\
 % 3030.58828 &    -40901.70 &            2.31 &  -40886.79 &          8.00 &  -40900.07 &          3.94 &  -40903.84 &          3.20 &          615.83 &            2196.43 &        3.25 &           0.01 &       0.01 &          0.01 \\
 % 3031.56744 &    -40907.58 &            2.38 &  -40906.26 &          7.66 &  -40909.81 &          3.92 &  -40907.34 &          3.46 &         6966.69 &            2229.48 &        3.25 &           0.01 &       0.00 &          0.01 \\
 % 3035.59686 &    -40902.29 &            3.80 &  -40891.47 &         13.76 &  -40905.49 &          6.78 &  -40903.48 &          5.00 &        -9199.59 &            3528.79 &        3.23 &           0.02 &      -0.01 &          0.02 \\
 % 3037.56491 &    -40903.73 &            2.29 &  -40898.83 &          8.07 &  -40905.53 &          3.94 &  -40903.07 &          3.12 &          643.21 &            2188.33 &        3.26 &           0.01 &      -0.00 &          0.01 \\
 % 3040.54178 &    -40899.60 &            1.97 &  -40887.23 &          5.45 &  -40905.29 &          3.07 &  -40899.85 &          3.21 &        13514.91 &            1797.66 &        3.26 &           0.01 &       0.01 &          0.01 \\
 % 3041.55272 &    -40901.04 &            2.09 &  -40889.80 &          7.07 &  -40907.06 &          3.51 &  -40899.53 &          2.93 &         5072.08 &            1982.92 &        3.25 &           0.01 &       0.00 &          0.01 \\
 % 3045.60561 &    -40896.99 &            5.01 &  -40893.91 &         16.28 &  -40900.54 &          9.05 &  -40895.25 &          6.66 &         4700.07 &            4455.02 &        3.22 &           0.02 &      -0.02 &          0.02 \\
 % 3046.55768 &    -40896.38 &            6.75 &  -40890.16 &         18.63 &  -40909.07 &         12.68 &  -40900.29 &          9.05 &        24042.02 &            5585.02 &        3.28 &           0.04 &      -0.03 &          0.04 \\
 % 3048.54503 &    -40897.59 &            2.26 &  -40899.58 &          7.38 &  -40902.10 &          3.73 &  -40893.68 &          3.24 &        11267.01 &            2125.62 &        3.27 &           0.01 &       0.01 &          0.01 \\
 % 3049.50934 &    -40900.78 &            2.48 &  -40887.20 &          7.75 &  -40904.77 &          4.02 &  -40900.24 &          3.66 &         9538.95 &            2313.08 &        3.28 &           0.01 &       0.01 &          0.01 \\
 % 3051.52528 &    -40900.40 &            2.64 &  -40893.35 &          9.63 &  -40899.09 &          4.59 &  -40900.68 &          3.56 &         2775.74 &            2518.47 &        3.28 &           0.01 &       0.01 &          0.01 \\
\bottomrule
\end{tabular}
\end{table*}
\end{landscape}


==> table_timeseries_tmp.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
{} &          bjd &         rv &       erv &      fwhm &        bis &    Halpha &      NaD1 &      NaD2 \\
\midrule
0  &  1985.480409 &   2.914881 &  2.349646 &  3.025786 &  -9.140980 &  0.876768 &  0.439504 &  0.570434 \\
1  &  1986.451684 &   2.170591 &  1.327641 &  3.048638 & -12.933950 &  0.880400 &  0.428430 &  0.561318 \\
2  &  1987.422057 &   1.103092 &  2.006567 &  3.038358 &  -4.711400 &  0.887566 &  0.421716 &  0.561281 \\
3  &  1988.506267 &   0.713112 &  2.220544 &  3.001679 & -10.231320 &  0.884743 &  0.436879 &  0.582787 \\
4  &  1989.506477 &  -6.092720 &  2.836951 &  3.057358 &   1.766286 &  0.883537 &  0.446227 &  0.580861 \\
5  &  1990.529416 &   4.462411 &  1.852999 &  3.098760 & -20.094320 &  0.885119 &  0.438042 &  0.574438 \\
6  &  1993.462305 &   4.207264 &  3.777883 &  3.081392 & -20.140290 &  0.880430 &  0.480519 &  0.614600 \\
7  &  2007.433332 &   1.401103 &  1.213877 &  3.111467 &  -7.234580 &  0.890907 &  0.421580 &  0.557331 \\
8  &  2008.457941 &   1.478451 &  1.455552 &  3.091279 &  -5.541900 &  0.886646 &  0.420563 &  0.559306 \\
9  &  2019.432121 &  -1.197287 &  1.696500 &  3.082221 & -18.423510 &  0.871353 &  0.427308 &  0.567422 \\
10 &  2026.417263 &  -1.508788 &  1.837150 &  3.083658 &  -7.530990 &  0.873630 &  0.434181 &  0.577184 \\
11 &  2027.416684 &   3.050822 &  1.590788 &  3.148105 &  -1.615810 &  0.878386 &  0.429410 &  0.570225 \\
12 &  2028.462885 &  -2.993618 &  1.629545 &  3.068003 &  -9.554550 &  0.872590 &  0.421865 &  0.561168 \\
13 &  2235.741744 &   3.546687 &  1.804781 &  3.058168 &  -7.196470 &  0.893712 &  0.434418 &  0.578162 \\
14 &  2236.701498 &  -0.145987 &  1.772264 &  3.044550 &   1.495609 &  0.895609 &  0.432002 &  0.577339 \\
15 &  2237.780558 &  -5.731083 &  4.719089 &  3.004831 & -14.355270 &  0.895084 &  0.456872 &  0.571398 \\
16 &  2239.735213 &   0.715179 &  1.303199 &  3.052813 &  -8.073650 &  0.887784 &  0.424777 &  0.558535 \\
17 &  2240.763206 &   1.845368 &  1.452400 &  3.038714 &  -3.763210 &  0.886943 &  0.418707 &  0.557022 \\
18 &  2244.695698 &   5.317866 &  1.267387 &  3.066781 &  -6.885480 &  0.891000 &  0.422465 &  0.562751 \\
19 &  2246.732253 &   0.639424 &  3.077508 &  3.071838 & -33.782000 &  0.884534 &  0.507512 &  0.602586 \\
20 &  2248.684464 &  -4.515321 &  1.645052 &  3.056177 & -10.564490 &  0.888306 &  0.423189 &  0.568242 \\
21 &  2253.785194 &  -3.849447 &  1.485134 &  3.073445 &  -6.738270 &  0.898069 &  0.431088 &  0.571274 \\
22 &  2255.742590 &  -1.853580 &  2.333925 &  3.012585 & -17.809360 &  0.893487 &  0.435818 &  0.566350 \\
23 &  2256.749713 &   1.309662 &  2.057892 &  3.058646 &  -5.820290 &  0.902477 &  0.456740 &  0.565016 \\
24 &  2267.764207 &   0.293798 &  1.846558 &  3.009532 & -10.491520 &  0.888664 &  0.439856 &  0.571146 \\
25 &  2268.673971 &   1.035207 &  2.134417 &  3.078157 &  -9.656040 &  0.886054 &  0.442069 &  0.578663 \\
26 &  2272.625601 &  -1.133653 &  1.573375 &  3.053512 &  -3.067120 &  0.891441 &  0.430611 &  0.565091 \\
27 &  2275.615295 &  -0.943361 &  1.502329 &  3.093230 &  -0.916210 &  0.891273 &  0.433540 &  0.566222 \\
28 &  2276.660052 &   2.971039 &  1.556139 &  3.081245 &  -9.150400 &  0.890619 &  0.435934 &  0.560728 \\
29 &  2277.694138 &   7.212189 &  1.813598 &  3.063018 & -11.798230 &  0.891410 &  0.430218 &  0.565716 \\
30 &  2288.704342 &   4.627531 &  1.735527 &  3.027571 & -12.752500 &  0.902190 &  0.422233 &  0.560339 \\
31 &  2289.607691 &   0.240488 &  1.236495 &  3.060853 &  -7.966770 &  0.894817 &  0.427650 &  0.557962 \\
32 &  2298.513138 &   4.499006 &  3.412182 &  3.053069 & -23.293670 &  0.885859 &  0.466218 &  0.620264 \\
33 &  2299.705456 &  -0.366764 &  2.519298 &  3.019713 & -18.885570 &  0.897153 &  0.465743 &  0.589715 \\
34 &  2304.631724 &   6.529311 &  3.787311 &  3.025803 &   9.454084 &  0.898763 &  0.463209 &  0.595788 \\
35 &  2306.571410 &  -9.058994 &  6.446400 &  3.057451 &  -9.112540 &  0.900645 &  0.518708 &  0.613535 \\
36 &  2307.539874 &   5.014078 &  1.753499 &  2.977886 & -11.321140 &  0.894030 &  0.427862 &  0.559956 \\
37 &  2309.528293 &   4.270002 &  2.425806 &  2.994353 & -15.334160 &  0.894094 &  0.440011 &  0.574570 \\
38 &  2310.495286 &   7.481029 &  3.058062 &  2.978863 &  -3.261130 &  0.899640 &  0.463816 &  0.581867 \\
39 &  2323.622313 &  -5.380628 &  2.033833 &  3.059397 &  -8.297690 &  0.884135 &  0.443787 &  0.582814 \\
40 &  2326.554394 &  -2.170825 &  1.425171 &  3.121644 &  -2.817070 &  0.882192 &  0.428383 &  0.566080 \\
41 &  2327.504992 &  -2.706617 &  1.621222 &  3.044799 &  -5.990480 &  0.887690 &  0.425568 &  0.568942 \\
42 &  2328.557784 &  -0.164639 &  2.833013 &  3.011220 &  -6.942400 &  0.883902 &  0.445240 &  0.581973 \\
43 &  2330.665706 &   4.918363 &  1.814926 &  3.012213 & -12.689570 &  0.882228 &  0.451421 &  0.583409 \\
44 &  2332.646479 &  -0.075104 &  2.635807 &  3.015142 & -11.828530 &  0.886883 &  0.457887 &  0.588762 \\
45 &  2333.666771 &   2.004803 &  1.883653 &  3.023775 & -16.561250 &  0.883934 &  0.436197 &  0.576036 \\
46 &  2343.593708 &   6.042332 &  3.209578 &  2.989143 &  -6.952520 &  0.888297 &  0.465649 &  0.593042 \\
47 &  2344.631185 &   7.937559 &  3.121573 &  2.954609 &   9.170382 &  0.897243 &  0.448043 &  0.584799 \\
48 &  2345.496331 &   5.244962 &  3.503492 &  2.960451 & -16.348030 &  0.887856 &  0.434906 &  0.570786 \\
49 &  2353.449225 &   0.300061 &  2.221026 &  3.054535 &  -3.247170 &  0.889294 &  0.446506 &  0.592182 \\
50 &  2353.516513 &   3.146984 &  1.642773 &  3.061811 &  -9.862070 &  0.878844 &  0.432584 &  0.576727 \\
51 &  2360.539634 &   1.864041 &  2.602369 &  3.016233 &  -4.184780 &  0.882202 &  0.446140 &  0.579093 \\
52 &  2363.540761 &   1.766689 &  2.195386 &  3.040613 &  -7.865310 &  0.884453 &  0.423495 &  0.551304 \\
53 &  2364.536608 &   1.239232 &  2.040855 &  3.059685 &  -7.317790 &  0.887300 &  0.420997 &  0.568515 \\
54 &  2365.521657 &   1.854769 &  2.087801 &  3.040803 &  -9.755030 &  0.880513 &  0.419855 &  0.557151 \\
55 &  2366.537827 &  -3.308982 &  1.403145 &  3.048514 &  -5.991680 &  0.887816 &  0.413802 &  0.559173 \\
56 &  2367.504903 &  -2.444993 &  1.352251 &  3.075844 &  -9.332660 &  0.886753 &  0.410966 &  0.552322 \\
57 &  2368.436714 &   0.075104 &  1.508389 &  3.027093 &  -4.499190 &  0.885187 &  0.417792 &  0.549130 \\
58 &  2370.475479 &  -5.219963 &  3.786697 &  3.091475 &  -2.348240 &  0.878765 &  0.453085 &  0.605767 \\
59 &  2370.495860 &  -6.179669 &  2.522098 &  3.056671 &  -0.968930 &  0.884006 &  0.448455 &  0.582771 \\
60 &  2377.474846 &   0.262045 &  2.114091 &  3.054530 &  -3.556150 &  0.888530 &  0.435011 &  0.578775 \\
61 &  2378.442734 &  -1.620481 &  1.839394 &  3.033044 & -12.071010 &  0.884758 &  0.419174 &  0.572700 \\
62 &  2379.446061 &  -0.146151 &  1.790252 &  3.060932 &  -7.268430 &  0.882592 &  0.427484 &  0.588081 \\
63 &  2387.408790 &  -3.805790 &  1.728308 &  3.073986 & -10.053810 &  0.891807 &  0.416748 &  0.560981 \\
64 &  2388.438694 &   1.222392 &  1.367733 &  3.060614 &  -3.309150 &  0.889907 &  0.416398 &  0.554237 \\
65 &  2390.429835 & -13.402415 &  1.993990 &  3.061745 &  -2.996360 &  0.877455 &  0.424469 &  0.555810 \\
66 &  2391.440493 &  -4.972614 &  1.863493 &  3.040621 &   6.305203 &  0.880754 &  0.415675 &  0.566135 \\
67 &  2392.426545 &  -0.988207 &  1.092804 &  3.060456 & -10.436920 &  0.879837 &  0.423297 &  0.566702 \\
68 &  2393.437910 &  -0.521344 &  1.854616 &  3.089095 & -13.396530 &  0.880763 &  0.427524 &  0.573022 \\
69 &  2394.421012 &   0.614272 &  1.542419 &  3.060506 & -11.554370 &  0.906010 &  0.431694 &  0.563162 \\
70 &  2414.374025 &   2.884332 &  2.125472 &  3.047879 &  -2.958540 &  0.874229 &  0.513691 &  0.631304 \\
71 &  2415.403897 &  -1.461467 &  1.711457 &  3.057170 &  -3.670770 &  0.880057 &  0.428488 &  0.573900 \\
72 &  2416.380450 &   1.614000 &  1.178886 &  3.077775 &  -6.259520 &  0.876630 &  0.424537 &  0.559920 \\
73 &  2642.701745 &  -0.884599 &  1.902406 &  3.061193 &  -4.410780 &  0.866789 &  0.442955 &  0.581261 \\
74 &  2648.666996 &  -4.456283 &  1.812632 &  3.048515 &  -1.677440 &  0.867059 &  0.447249 &  0.582831 \\
75 &  2649.566437 &  -2.876102 &  1.558242 &  3.079524 &  -8.906320 &  0.859797 &  0.441963 &  0.563480 \\
76 &  2651.672013 &  -6.077616 &  1.194029 &  3.071556 &  -8.188770 &  0.861883 &  0.425149 &  0.565754 \\
77 &  2659.664794 &   4.033377 &  1.213544 &  3.088356 &  -4.944170 &  0.869120 &  0.421413 &  0.559340 \\
78 &  2682.540311 &   2.982620 &  1.833903 &  3.087754 &  -0.521530 &  0.861789 &  0.422278 &  0.564922 \\
79 &  2686.569209 &  -2.078644 &  3.658178 &  3.087889 & -18.335260 &  0.847056 &  0.510187 &  0.623748 \\
80 &  2690.645448 &  -0.920834 &  2.518819 &  3.014021 &  -2.680140 &  0.860554 &  0.447861 &  0.563392 \\
81 &  2705.614036 &  -4.717027 &  1.991208 &  3.050583 & -14.635170 &  0.863603 &  0.431307 &  0.565567 \\
82 &  2706.557606 &  -6.779250 &  1.791192 &  3.088729 &  -6.992790 &  0.866294 &  0.430412 &  0.568423 \\
83 &  2707.548164 &  -9.406405 &  1.831950 &  3.066550 & -12.427450 &  0.864587 &  0.424888 &  0.565864 \\
84 &  2708.502959 & -12.307447 &  2.816623 &  3.061122 &  -4.339870 &  0.864299 &  0.460272 &  0.596853 \\
85 &  2709.437755 &  -2.300939 &  2.507303 &  3.044798 &  -6.362780 &  0.865636 &  0.443822 &  0.575369 \\
86 &  2712.537130 &  -8.416674 &  2.455885 &  3.064928 &   1.575124 &  0.875665 &  0.443877 &  0.585025 \\
87 &  2714.567698 &  -1.210222 &  1.799317 &  3.071562 &  -9.432570 &  0.875449 &  0.427377 &  0.565593 \\
88 &  2715.543441 &  -1.884365 &  1.749886 &  3.106259 &  -2.214400 &  0.887327 &  0.435315 &  0.569122 \\
89 &  2716.533651 &  -5.548784 &  1.503164 &  3.052901 &  -7.852500 &  0.882180 &  0.419117 &  0.556032 \\
90 &  2717.519474 &  -4.649235 &  1.034350 &  3.082438 &  -0.201420 &  0.888269 &  0.413149 &  0.561874 \\
91 &  2718.492972 &   0.552234 &  1.221192 &  3.067364 &  -3.302860 &  0.883136 &  0.411564 &  0.557754 \\
\bottomrule
\end{tabular}

